Enhancing Next Destination Prediction: A Novel Long Short-Term Memory Neural Network Approach Using Real-World Airline Data

In the modern transportation industry, accurate prediction of travelers' next destinations brings multiple benefits to companies, such as customer satisfaction and targeted marketing. This study focuses on developing a precise model that captures the sequential patterns and dependencies in travel data, enabling accurate predictions of individual travelers' future destinations. To achieve this, a novel model architecture with a sliding window approach based on Long Short-Term Memory (LSTM) is proposed for destination prediction in the transportation industry. The experimental results highlight satisfactory performance and high scores achieved by the proposed model across different data sizes and performance metrics. This research contributes to advancing destination prediction methods, empowering companies to deliver personalized recommendations and optimize customer experiences in the dynamic travel landscape.

==> aff.tex <==
\author{Salih Salihoglu \orcidicon{0000-0002-3424-8587}\,, Gulser Koksal\orcidicon{0000-0002-8005-2120}\,, and Orhan Abar \orcidicon{0000-0003-4362-1395}\,
\thanks{This paragraph of the first footnote will contain the date on which
you submitted your paper for review. It will also contain support information,
including sponsor and financial support acknowledgment.}
\thanks{Salih Salihoglu is with the Department of Industrial Engineering, Middle East Technical University, Ankara, Turkey (e-mail:salih_245@hotmail.com).}
\thanks{Gulser Koksal is with the Department of Industrial Engineering, Middle East Technical University, Ankara, Turkey (e-mail:pxp136@med.miami.edu).}
\thanks{Orhan Abar is with the Department of Computer Engineering, Osmaniye Korkut Ata University, Osmaniye, Turkey (e-mail:e.celik@miami.edu).}}

